Per Garment Capture and Synthesis for Real-time Virtual Try-on

Virtual try-on is a promising application of computer graphics and human computer interaction that can have a profound real-world impact especially during this pandemic. Existing image-based works try to synthesize a try-on image from a single image of a target garment, but it inherently limits the ability to react to possible interactions. It is difficult to reproduce the change of wrinkles caused by pose and body size change, as well as pulling and stretching of the garment by hand. In this paper, we propose an alternative per garment capture and synthesis workflow to handle such rich interactions by training the model with many systematically captured images. Our workflow is composed of two parts: garment capturing and clothed person image synthesis. We designed an actuated mannequin and an efficient capturing process that collects the detailed deformations of the target garments under diverse body sizes and poses. Furthermore, we proposed to use a custom-designed measurement garment, and we captured paired images of the measurement garment and the target garments. We then learn a mapping between the measurement garment and the target garments using deep image-to-image translation. The customer can then try on the target garments interactively during online shopping.

==> content/05-acq.tex <==
\section{Garment capturing}\label{sec:data_collection}
\subsection{Capturing device - Actuated Mannequin}
We designed the basic body shape of our actuated mannequin that approximates the average male body shapes in a commonly used parametric body shape model SMPL~\cite{loper2015smpl}.
% We matched the parameters of the model such that it approximates the local average body shape of men.
To enable the mannequin to pose for a large variety of motions commonly found during physical try-out sessions in a physical store, we equipped it with nine degrees-of-freedoms:
\begin{itemize}
    \item independent arm movement for both arms
    \item four adjustable body region
    \item rotation around the center
\end{itemize}

More specifically, the torso is segmented into four adjustable regions, with three front-facing actuators and one side-facing actuator (\figname~\ref{fig:man_dofs}(a)).
And each upper arm is actuated with two servo motors, allowing movement along the yaw and pitch axes (\figname~\ref{fig:man_dofs}(b) and (c)).
All motors can be controlled independently and connected to the host computer, enabling automatic capturing.
The mannequin's arms and outer shell are 3D printed which is easy for reproduction, and it is strengthened with sheet metal internally.
We plan to release the design so that the actuated mannequin can be reproduced.

% \begin{figure}[h]
% \begin{center}
% \captionsetup{type=figure}
%   \includegraphics[width=\linewidth]{figures/arm_image.png}
%   \caption{
%   \iccmt{Can we merge the content of this figure with other figure illustrates the mannequin?}
%   We have designed a easily detachable arm system to facilitate putting on and removing garment. 
% %   The arms are attached only via magnet and we have three screws to align the orientation.
%   }
% \label{fig:arm}
% \end{center}
% \end{figure}

\begin{figure*}[t!]
    \centering
        \includegraphics[width=\linewidth]{figures/manniquinn_dof.jpeg}
    \caption{
Actuated mannequin degree-of-freedoms.
(a) The torso of our actuated mannequin is segmented into four adjustable regions (illustrated in red arrows), with three front-facing actuators and one side-facing actuator.
(b) (c) And each upper arm is actuated with two servo motors, allowing movement along the yaw and pitch axes.
}
\label{fig:man_dofs}
\end{figure*}

The mannequin is placed in front of a single color background, and we used an RGBD camera (Microsoft Azure Kinect DK) with fixed focal length, shutter speed, and exposure setting during capturing and testing.
We used color-based segmentation for separating the garment and the body parts; hence we avoid using the color of the background that is similar to the one of the target garment.
During our capturing, we used a black background for all the target garments and the measurement garment. 
We also dress the mannequin in a full-body skin-tight suit in the same color as the background.
The reason is that the surfaces of the mannequin generate reflections inference with the color-based garment segmentation.
In addition, the arm modules are detachable to allow garment changing.

\subsection{Capturing process}
To generate the virtual try-on result for each target garment, the retailer must capture data for both the target garments and a measurement garment (we will describe the design of the measurement garment in \secname~\ref{subsec:measurment_design}). 
However, measurement garment data can be reused to pair up with any new target garment the retailer wants to capture.
Thus, the retailer only needs to capture the measurement garment only once.
The procedure for capturing the measurement garment and the target garments are identical.
To capture a piece of garment, we first dress the mannequin in a skin-tight suit and set up a black background screen.
% of the same color. 
% We have three colors of undergarments and background screen available, black, white, and green. 
% We choose the undergarment and background color by avoiding colors on the target garment we are capturing. 
Afterward, we dress up the mannequin in the garment and begin the capturing session. 

We capture the garment by rotating the mannequin in a fixed body configuration (i.e., body size and arm pose). 
With our current setup, we collect $1$ image each degree the mannequin is rotated, and we captured $\pm67^{\circ}$ from the front of the mannequin. 
We divided the arms' movement range into two $5x5$ grids uniformly, and we moved both arms uniformly sampled from the grids. 
We adjusted the size of the body by $1cm$ both horizontally and vertically as we finish capturing a rotation, cycling through a predefined limit (0\~20cm). 
In total, we collected $84,375$ RGBD images for each piece of garment.
The entire process is automated except the initial setup and takes approximately $2$ hours for each piece of garment. 

\subsection{Data post-processing}\label{subsec:post_processing}
After capturing each target garment, we segmented the garment out from the background and obtain a garment mask by thresholding the depth values first and further refining the mask through color thresholding in HSV color space.
% Up until here, the capturing and processing for measurement garment and target garment are identical. 
To align a pair of both the measurement garment and a target garment
% For a pair of images for measurement garment and target garment 
under identical viewing angle and body configuration, we first crop the measurement garment using the garment mask.
The mask of the measurement garment always maintains a fix-sized border at the top and bottom relative to the height of the garment mask. 
We apply identical cropping parameters to the target garment to generate a direct match. 
Finally, we resized the images to $512px\times512px$ for learning.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/comparison_result2.png}
  \caption{
%   \iccmt{Update the caption.}
  Our try-on results on various target garments.
  Given the frame of input motion, our method synthesize results with clearer garment and body parts.
  We showed the ground truth in the last column for reference.
%   (a) Reference images of garments tested with our system. From the left, Measurement garment, knitted sweater, single colored T-shirt, Kimono (Traditional Japanese garment), and printed T-shirt. (b) The actor wearing measurement garment and the corresponding virtual try-on result using our system. (c) The actor wearing the target garment for reference.
}
\label{fig:target_garments_result}
\end{figure*}


%%%%
% Moreover, we designed the arm modules with various arm lengthes so that when we capture the garments with different sleeve lengthes, it will not be occluded as little as possible but still remain the geometry of the arm (\figname~\ref{}).
% \paragraph{Camera}
% We use a Microsoft Azure Kinect DK for image capturing. We fixed the focus length, shutter speed, and exposure settings during capturing and testing. We stored both the RGB as well as the depth image during the garment capturing sessions to facilitate the background removal for the training data. 

% To generate virtual try-on for one target garment, it is currently required to capture data for both the target garment as well as the measurement garment. However, the data of the measurement garment can be reused for new target garment. 
% The procedure for capturing the garments are identical but are subjected to slightly different post-processing. 

==> content/06-capturing_system.tex <==
\section{Capturing system}\label{sec:capturing_system}
\subsection{Actuated Mannequin}
The actuated mannequin has nine degrees-of-freedom: rotation around the center, independent arm movement for both arms along the roll and pitch axis, and four adjustable body region (\figname~\ref{}). 
It allows the robot to pose for a large variety of motions commonly found during physical try-out sessions in phyiscal store.

Each upper arm is actuated with two servo motors, allowing movement along the yaw and pitch axes. 

The torso is segmented into four adjustable regions, with three front-facing actuators and one side-facing actuator, each can be controlled independently.  

The mannequin arms are actuated by four servo motors corresponding to each joint movement and the turntable contains a single motor. All motors are connected to the host computer.
We designed the shape of the actuated mannequin based on SMPL~\cite{loper2015smpl}, a parameterized body model, we matched the parameters of the model such that it approximates the local average body shape of men. 
The arms and outer shell of the mannequin are 3D printed and is strengthen with sheet metal internally.

%\begin{figure}[h]
\begin{center}
\captionsetup{type=figure}
  \includegraphics[width=\linewidth]{figures/arm_image.png}
  \caption{We have designed a easily detachable arm system to facilitate putting on and removing garment. The arms are attached only via magnet and we have three screws to align the orientation.}
\label{fig:arm}
\end{center}
%\end{figure}

The mannequin is placed in front of a single color background and a camera is placed in front of the mannequin. We used color-based segmentation for the garment, hence we avoid using the color of the background that is similar to the one of the target garment. In our study, we used green background for all the target garment and used black background for the measurement garment. We also dress the mannequin with a full body skin-tight suit in the same color as the background.
In addition, we designed a detachable arm module with various arm length such that the garment is occluded as little as possible. 
%\begin{figure}[h]

%\end{figure}



\subsection{Camera}
We use a Microsoft Azure Kinect DK for image capturing. We fixed the focus length, shutter speed, and exposure settings during capturing and testing. We stored both the RGB as well as the depth image during the garment capturing sessions to facilitate the background removal for the training data. 




%\begin{figure}[h]
\begin{center}
\captionsetup{type=figure}

% \begin{figure*}
%  \centering
 \includegraphics[width=\linewidth]{figures/measurement_garments.png}
 \caption{
     Measurement garments. (a) segmentation garment, (b) checkerboard garment, (c) dot garment, (d) color gradient garment. For (b) and (c) the front and back are identical.
 }
 \label{fig:tshirt}
% \end{figure*}
\end{center}
%\end{figure}



==> content/07-data.tex <==
\section{Data acquisition and post-processing}\label{sec:data_collection}
To generate virtual try-on for one target garment, it is currently required to capture data for both the target garment as well as the measurement garment. However, the data of the measurement garment can be reused for new target garment. 
The procedure for capturing the garments are identical but are subjected to slightly different post-processing. 

\subsection{Capturing method}
To capture a piece of garment, we first dress the mannequin with a single-colored undergarment, as well as setting up a background screen of the same color. 
We have three color of undergarments and background screen available, black, white, and green. 
We choose the color of the undergarment and background by avoiding colors that is on the garment we are capturing. 
Afterward, we dress up the mannequin in the garment and begin the capturing session. 
We adjust and fix the camera color control parameter manually to ensure the garment is captured properly.

We capture the garment by rotating the mannequin in a fixed body configuration (i.e., body size and arm pose). 
With our current setup, we collect $1$ image each degree the mannequin is rotated and we captured $\pm67^{\circ}$ from front of the mannequin. 
We divided the movement range of the arms into two $8x8$ grids for each of the arms, and uniformly sampled from the grids. 
We adjusted the shape of the body by $1cm$ incremental both horizontally and vertically as we finish capturing a rotation, cycling through a predefined limit (0~20cm). 
In total we collected $184,320$ images for each piece of garment.

The entire process is automated except the initial setup and takes approximately $2$ hours for each piece of garment. 
We decided on the data collection protocol experimentally.

\subsection{Post-processing}\label{subsec:post_processing}
After capturing each target garment, we extracted a garment mask from the captured images by thresholding their depth values.
In addition, we apply color thresholding in HSV color space to the image to refine the segmentation. 

Up until here, the capturing and processing for measurement garment and target garment are identical. For a pair of images for measurement garment and target garment under identical viewing angle and body configuration, we first crop the measurement garment using the garment mask such that the mask of the measurement garment always maintain a fix-sized borders at the top and bottom relative to the height of the garment mask. We apply identical cropping parameters to the target garment to generate a direct match. 
Finally, the images are resized to $512px$ for learning.


\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/garment_gallery.png}
  \caption{(a) Reference images of garments tested with our system. From the left, Measurement garment, knitted sweater, single colored T-shirt, Kimono (Traditional Japanese garment), and printed T-shirt. (b) The actor wearing measurement garment and the corresponding virtual try-on result using our system. (c) The actor wearing the target garment for reference.}
\label{fig:target_garments}
\end{figure*}



==> content/08-mapping.tex <==
\section{Synthesis and Try-on}
\label{sec:method}
Figure~\ref{fig:overview} details the workflow of the synthesis system. 
Taking the images of measurement and training garment as training data, we train an image-to-image translation network for each measurement garment and target garment pair. 

% %\begin{figure}[h]
% \begin{center}
% \captionsetup{type=figure}
%  \includegraphics[width=\linewidth]{figures/measurement_garments.png}
%  \caption{
%      Measurement garments. (a) segmentation garment, (b) checkerboard garment, (c) dot garment, (d) color gradient garment. For (b) and (c) the front and back are identical.
%  }
%  \label{fig:tshirt}
% \end{center}

\subsection{Measurement garment design}
\label{subsec:measurment_design}
One of the major differences between our system and many existing virtual try-on systems is that we ask the user to wear a measurement garment during the interaction.
By defining the problem as an image-to-image translation from
measurement to target garment, we can capture rich garment deformations (wrinkles) of measurement garment during try-on and transfer it to target garment.
Custom design measurement garment also makes image segmentation problem tractable, enabling real-time interaction.
% The main purpose of this design is to provide a fast trackable and easy-to-segment body representation.
Hence, there are several requirements for the design of the measurement garment. 
First, it should be separable from the customer's body (skin color) computationally efficient and robust under dramatic deformations.
Second, it should convey the body configuration (posture and size) of a customer. 
Third, it should allow the image-to-image translation network to easily translate it to a wide range of target garments without introducing additional artifacts. 

To address the above requirements, 
we have designed a segmentation garment inspired by segmentation visualization result. 
We concluded that the segmentation garment is effective for synthesizing realistic and stable virtual try-on result, since the segmentation garment effectively divided the input image into multiple patches, thus allows the learning to perform more efficiently. 
In addition, by using a one-hot representation allows our garment extraction process to run at a much lower resolution, without compromising the image generation quality. 
% , which is inspired by the visualization of the segmentation map, outperforms the rest of the measurement garments. 


% We designed and tested various patterns including, 
% \begin{itemize}
%     \item Single color, no pattern (plain),
%     \item Color coded, discrete segmentation (segmentation),
%     \item Color coded, gradient image (gradient),
%     \item monochrome, checkerboard pattern (checkerboard),
%     \item monochrome, dot pattern (dot).
% \end{itemize}
% Please see figure~\ref{fig:tshirt} for a gallery of the measurement garments we designed and tested. In our initial testing, we found that the segmentation garment outperformed the rest of the garment and we used the segmentation suit for all of our experiment.


\subsection{Image-to-image translation}
We learned the mapping between the measurement garment and each of the target garment using image-to-image translation with the specific architecture borrowed from Pix2PixHD~\cite{wang2018pix2pixHD}. For each target garment, we use all the $184,320$ images captured for training, and we train a new network for each measurement/target garment pair. 
We augmented the input image using standard image augmentation techniques, including random affine transform and minor color jittering. 
We applied a random translation of $±50px$ at each direction, random rotation within $±15°$, shearing for $±10°$. 
We also applied change of saturation, hue, brightness, and contrast for $0.05$. 
We used the default parameters provided by Pix2PixHD without hyperparameter tuning. 
We trained the system for six epoch, which took approximately five days on a single RTX 2080Ti.

\subsection{Try-on}
During the interaction stage, a customer wearing the measurement garment and stand in front of our system. 
%goes into the fitting room. 
% We adjust the camera height to match capturing setting. 
Generating the try-on result contains three stages: measurement garment extraction, target garment inference, and final composition (as shown in the upper row in \figname~\ref{fig:overview}). 

\paragraph{Measurement garment extraction}
% \label{subsec:garment_extract}
% We have designed a measurement garment that is easy to extract from a virtual try-on setting. The most recent version of the measurement garment contains eight color blocks inspired by 3D dense pose registration visualization.
The system extracts the garment from the input camera feed using a three-step process. 
A rough whole body mask is first generated using the depth information. 
We then applied skin detection to the image, which removes the exposed arm, face, and neck of the user and leaves only the garment in the image. 
The garment is then segmented into the eight color patches using K-Means clustering in HSV color space. 

\paragraph{Target garment inference}
After extracting the garment mask, we cropped the frame using the cropping parameters chosen at \secname~\ref{subsec:post_processing}. 
The cropped image is then masked with the garment mask and used as the input to the image-to-image translation model to infer the resulted target garment. 

\paragraph{Final re-composition}
The output result of the image-to-image translation model is then re-composed back into the original frame. 
We do so by first applying the post-processing (cropping and resizing) in reverse order. 
We automatically generated a garment mask from the network output using the intensity value to avoid overlay body regions that should not be covered.
Currently, we assume the garment should be always on top and should remain only one single component.
So if the arm stays on top of the garment that separate the garment into two parts, our method currently fails to map the target garment to the measurement garment.
% Re-composing the entire output from the image-to-image translation model will overlay other body regions that should not be covered; therefore, we 
% Currently, we use the segmentation map produced in the first try-on step to ensure that the arms are always on top of the garment. 

%%%
% During data acquisition (Sec. \ref{sec:data_collection}), the retailer first puts a measurement garment on the mannequin. The system then takes pictures of the mannequin in diverse body poses and shape. The system then performs segmentation to remove the background from the captured images. The same process applied to a target garment. 

%Third, it should be free from other factors that varies between the data acquisition time and the test time such as self occlusion. 

% The customer wears a measurement garment at test time. 
% Scholz~\etal~\shortcite{scholz2005garment} developed and evaluated different patterns such as checkerboard, random color dots for garment motion capture.

% It is our future work to test more variety of measurement garment designs and clarify the strength and limitations of each design.

% In execution time, a customer wears the measurement garment and stand in front of a camera. 
% The system then replaces the measurement garment with the target garment and shows the result in the display.
% In our experiments, each frame from the camera feed to the output takes in average $450$ milliseconds to compute, with the image-to-image translation taking up $190$ milliseconds in average (including preprocessing, GPU I/O, and composition), background removal, garment preprocessing and other image processing takes up the rest of the time. It is worth noting that our method does not require performing accurate 2D/3D skeleton registration by default. 

==> content/09-inference.tex <==
\section{Try-on}
At the execution stage, a customer wearing the measurement garment goes into the fitting room. We adjust the camera height to match capturing setting. The try-on process contains three stages, garment extraction, inference, and re-composition. 

\subsection{Garment extraction}\label{subsec:garment_extract}
We have designed a measurement garment that is easy to extract from a virtual try-on setting. The most recent version of the measurement garment contains eight color blocks inspired by 3D dense pose registration visualization.

The system extracts the garment from the input camera feed using a three-step process. A rough whole body mask is first generated using the depth information. We then applied skin detection on the image, which removes the exposed arm, face, and neck of the user and leaves only the garment in the frame. The garment is then further segmented into the eight color patches using K-Means clustering in HSV color space. 

\subsection{Inference}
After extracting garment mask, we cropped the frame using the garment mask and the cropping parameters chosen at Sec~\ref{subsec:post_processing}. The cropped image is then masked with the garment mask and is used as the input to the image-to-image translation model. 

\subsection{Re-composition}
The output result of the image-to-image translation model is then re-composed back into the original frame. We do so by first applying the post-processing (cropping and resizing) in reverse. Re-composing the entire output from the image-to-image translation model will overlay other body regions which should not be covered. Currently we use the segmentation map produced in Sec~\ref{subsec:garment_extract} to ensure that the arms are always on top of the garment. 

==> content/14-comparison.tex <==
\section{Comparison with image-based virtual try-on method}
We compare our method with a baseline image-based virtual try-on method. 

We designed five preset motions that are commonly found when trying a new piece of upper body garment. Motions recorded include \textbf{Turning} (rotating the torso), \textbf{Pulling} (stretching the garment), \textbf{Rowing a boat} (rotating the upper arms), \textbf{T-pose} (raising upper arms horizontally) and, \textbf{Zombie} (raising upper arms forward). Please refer Figure~\ref{fig:user_study_samples} for screenshots and supplemental material for the full videos. 


We designed $5$ motions asked the actors to perform a selection of actions and recorded their movement, the actors repeated the motions in all $5$ target garments in addition to the measurement garment. The recordings are processed offline using both our method and the baseline method. 

\subsection{Methods}
\subsubsection{Compare with image-based virtual try-on method}
We compared the following two virtual try-on methods in the study.
\begin{itemize}
    \item Our system (\textit{Ours})
    \item ACGPN, An existing image-based virtual try-on system  \cite{Yang_2020_CVPR} (\textit{Baseline})
\end{itemize}
%
\textit{Baseline} warps the input garment image to fit the pose of the body, whereas \textit{Ours} generates images based on the dataset contains many different poses taken using the mannequin. 
We chose \textit{Baseline} over other deep-image-based methods as it is the one highest image quality that we know of which provides a public implementation. Below we describe the difference for comparing the two methods.

Applying \textit{Baseline} for video virtual try-on can be done either animating a static picture of the actor using poses from the video frames (i.e., uses the pose of a static image as source and that of the current image as target) or treating each image from the video as the source (i.e., uses the same pose as source and target). We adopted the former method after testing both as it was more stable and demonstrated higher image quality. 
%
\textit{Ours} requires the user to wear the measurement garment and only uses the video frames instead. We explained the difference to the participants at the beginning of the study.
For \textit{Baseline}, we manually preprocessed the input videos (cropping and resizing to 192x256) to match the training data. For \textit{Ours} we cropped the video to remove excess background.

We note here that neither \textit{Baseline} or \textit{Ours} stabilised the network output using multiple frames, hence its a fair comparison.? 

%

%
Notice that our method is faster despite it runs at a much higher resolution $512x512$ vs \textit{Baseline} runs at $192x256$. However, in this study, the video is generated off-line frame-by-frame so the speed of the synthesis is not accounted for in the user study.

%
%After a 10 minutes break, the participants performed the 5 preset motions while wearing the 5 target garment and measurement garment. In total we record the 30 video clips of participants performing. We generated the virtual try-on result using our system and baseline for all 5 target garments, and combined it with the ground truth that is the participants themselves actually wearing the garment. The raw camera feed, result generated by the two systems, and the ground truth are put side by side to generate the final video. 
%
